Long-time predictive modeling of nonlinear dynamical systems using neural networks

We study the use of feedforward neural networks (FNN) to develop models of nonlinear dynamical systems from data. Emphasis is placed on predictions at long times, with limited data availability. Inspired by global stability analysis, and the observation of the strong correlation between the local error and the maximum singular value of the Jacobian of the ANN, we introduce Jacobian regularization in the loss function. This regularization suppresses the sensitivity of the prediction to the local error and is shown to improve accuracy and robustness. Comparison between the proposed approach and sparse polynomial regression is presented in numerical examples ranging from simple ODE systems to nonlinear PDE systems including vortex shedding behind a cylinder, and instability-driven buoyant mixing flow. Furthermore, limitations of feedforward neural networks are highlighted, especially when the training data does not include a low dimensional attractor. Strategies of data augmentation are presented as remedies to address these issues to a certain extent.

==> abstract.tex <==
%% abstract 
\begin{abstract}
%Despite the successful application of machine learning (ML) in fields such as image processing and speech recognition, progress toward employing ML to discover or represent the dynamics of complex physical systems has been relatively slow.  
We study the use of feedforward neural networks (FNN) to develop models of non-linear dynamical systems from data. Emphasis is placed on predictions at long times, with limited data availability. Inspired by global stability analysis, and the observation of strong correlation between the local error and the maximum singular value of the Jacobian of the FNN, we introduce Jacobian regularization in the loss function. This regularization suppresses the sensitivity of the prediction to the local error and is shown to improve accuracy and robustness. Comparisons are made between the proposed approach and sparse polynomial regression in examples ranging from simple ODE systems to nonlinear PDE systems including vortex shedding behind a cylinder, and instability-driven buoyant mixing flow. Furthermore, limitations of  feedforward neural networks are highlighted, especially when the training data does not include a low dimensional attractor. Strategies of data augmentation are presented as remedies to address these issues to a certain extent.
\end{abstract}


==> acknl.tex <==
\section*{Acknowledgments}

The authors gratefully acknowledge Zejia Zhang for proof-reading the paper and Professor Balaji Jayaraman for helpful discussion, comments and providing the POD data of two dimensional instability-driven buoyant mixing flows. This work was supported by AFOSR and AFRL under grants FA9550-16-1-0309 \& FA9550-17-1-0195.


==> bibgraphy.tex <==
\bibliographystyle{siamplain}
\bibliography{references}

==> vbe.tex <==
\subsection{Nonlinear PDE system: 1D viscous Burgers equation}\label{sec:vbe}

In this subsection we extend the problem from the reconstruction to the prediction with the one-dimensional viscous Burgers equation shown in \cref{eq:vbe}. The initial condition is generated randomly following a specific energy spectrum \cite{Parish2016} shown in \cref{eq:spectrum}. 
\begin{equation}{\label{eq:vbe}}
\frac{\partial  u}{\partial t} + u \frac{\partial u }{\partial x} = \nu \frac{\partial^2 u}{\partial x^2},
\end{equation}
where $x \in [0, 2\pi]$ with 2048 grid points uniformly distributed and $t\in[0, 20]$, $\nu=0.01$.

\begin{equation}{\label{eq:spectrum}}
    u(x,0) = \sum^{k_c}_{k=1} \dfrac{1}{\pi} \sqrt{2AE(k)} \sin(k x + \beta_k ),
\end{equation} where for each $k$, $\beta_k$ is a random number draw from a uniform distribution on $[-\pi, \pi]$, $E(k) = 5^{-5/3}$ if $1 \le k \ge 5$, $A=25$, and $E(k) = k^{-5/3}$ if $k > 5$. To fully resolve the system as a DNS, \ref{eq:vbe} is solved using a standard pseudo-spectral method with SSP-RK3 \cite{gottlieb2001strong} for time stepping. Here we choose $k_c = 2$. Discrete cosine transformation (DCT) is used to reduce the dimension of the full system to capture 4 cosine modes in the system where, on temporal average, around 97\% of kinetic energy is preserved. 

% description of the data 
Since the first component of DCT is constant, we can visualize the other three components in the feature space as shown in \cref{fig:vbe_train_feature_dist_and_lc_3d}. Note a very critical issue in modelling dynamical systems: initial data scarcity in high dimensional systems. Although the most dynamical system in nature contains some type of attractor (in current case a fixed point attractor due to viscosity) in the asymptotic sense, data scarcity is observed at the start of trajectory where the number of trajectories needed in order to provide enough information to cover the region of interest grows exponentially. Many previous works on applying neural-network based models for modelling dynamical systems \cite{tsung1995phase}\cite{Smaoui1997a}\cite{Wang2017} deal with problems on limiting cycles or chaotic attractors in a low-dimensional feature space where the issue of initial data scarcity is not significant or can be easily alleviated by a small increase in available data. However, for the purpose of modelling fluid dynamical systems when, initially, the state has not arrived at the low manifold attractor, data scarcity would shrink the generalizability of the model as feature dimension increases. Note that despite one of the benefits of a neural network is its linear growth of complexity with dimension of the system as opposed to traditional machine learning regression methods \cite{goodfellow2016deep}, initial data scarcity would limit its generalizability in modelling a high dimensional dynamical system that does not quickly fall on a low dimensional attractor. We believe this phenomenon also applies to other local machine learning models.

% 
To alleviate the initial data scarcity issue, we choose 18 trajectories from DNS results with different random number seed in the initial condition while keep the energy spectrum the same across all cases. Each trajectory contains states of 1000 snapshots equally spaced in time. For testing data, we simply consider one DNS result with an initial condition different from all training trajectories. The corresponding training and testing trajectories are presented in \cref{fig:vbe_train_feature_dist_and_lc_3d}.

% data distribution
\begin{figure}[htbp]
	\centering
	\includegraphics[width=\textwidth]{images/arranged/fig26}
	\caption{Feature distribution of training/testing data for component $x_2, x_3, x_4$. Left: with one training trajectory. Right: with 18 training trajectory. Black line: testing. Red line: training.}
	\label{fig:vbe_train_feature_dist_and_lc_3d}
\end{figure}


% % if we only use one trajectory, only poor result
% The resulting model is found to contain unacceptable large error near initial condition of testing trajectory and falls into a wrong attractor instead of approaching to the correct fixed point attractor. This is due to the sparsity of data at the transition phase. As seen in \cref{fig:vbe_train_feature_dist_and_lc_3d} the testing data is covered from $t=0$ to $20$. 


% % adding more trajectories helps, because if there are some trajectories near testing trajectory, the initial discrepancy will be pulled to attractor where model is confident about, but data scarcity issue still have if we extend the ...
% However, since we are dealing with a 4 dimension system instead of hundreds, a simple alleviation of initial data scarcity would be randomly adding more trajectories that generated from the same initial spectrum but with different random seeds. 

% training configuration
The basic model is trained with hyperparameters in \cref{table:hyperParameter_vbe_ann} with training epoch of 5000. The resulting learning curve and a posteriori evaluation are shown in \cref{fig:vbe_train_test_posteriori_ann}. Large error is observed near the initial states; this is due to initial data scarcity. It shows that error decreases once the trajectory falls on the fixed point attractor. 


\begin{figure}[htbp]
	\centering
	\includegraphics[width=\textwidth]{images/arranged/fig27}
	\caption{Result of basic model for one dimensional VBE turbulence case. Left: learning curve. Right: a posteriori result with augmented training trajectories. Red: $x_1$. Green: $x_2$. Blue: $x_3$. Cyan: $x_4$.}
	\label{fig:vbe_train_test_posteriori_ann}
\end{figure}


% \begin{figure}[htbp]
% 	\centering
% 	\includegraphics[width=\textwidth]{images/arranged/fig23}
% 	\caption{Data distribution of training/testing feature of 1D VBE, 4 POD modes case. From left to right, and top to bottom are $x_1$ vs $x_2$, $x_1$ vs $x_3$, $x_2$ vs $x_3$, $x_1$ vs $x_4$, $x_2$ vs $x_4$ and $x_3$ vs $x_4$ in sequence}
% 	\label{fig:vbe_train_feature_dist_and_lc}
% \end{figure}


% % fig: a posteriori on training data
% For training data with basic model configuration shown in \cref{table:hyperParameter_vbe_ann}, results are shown in \cref{fig:vbe_train_test_posteriori_ann}, as expected basic model successfully explains the variation in training data in a posteriori sense, i.e., given only the initial state.

\begin{table}[htbp]
\caption{Hyperparameter configuration of basic model: VBE system with four modes}
\label{table:hyperParameter_vbe_ann}
\centering
\begin{tabular}{|c|c|c|c|c|} \hline
		layer structure & activation function & loss function & optimizer & learning rate  \\ \hline
		4-30-30-30-4 & elu & MSE & Adam & 0.0005 \\  \hline
\end{tabular}
\end{table}

% 
% \begin{figure}[htbp]
% 	\centering
% 	\includegraphics[width=\textwidth]{images/arranged/fig24}
% 	\caption{A posteriori comparison between basic model and SINDy, 1D VBE, 4 DCT modes. Top: basic model. Bottom: SINDy. Left: training data. Right: testing data.}
% 	\label{fig:vbe_train_test_posteriori_ann}
% \end{figure}


